Correct-by-design Control Synthesis for Multilevel Converters using State Space Decomposition

High-power converters based on elementary switching cells are more and more used in the industry of power electronics owing to various advantages such as lower voltage stress and reduced power loss. However, the complexity of controlling such converters is a major challenge that the power manufacturing industry has to face with. The synthesis of industrial switching controllers relies today on heuristic rules and empiric simulation. The state of the system is not guaranteed to stay within the limits that are admissible for its correct electrical behavior. We show here how to apply a formal method in order to synthesize a correct-by-design control that guarantees that the power converter will always stay within a predefined safe zone of variations for its input parameters. The method is applied in order to synthesize a correct-by-design control for 5-level and 7-level power converters with a flying capacitor topology. We check the validity of our approach by numerical simulations for 5 and 7 levels. We also perform physical experimentations using a prototype built by SATIE laboratory for 5 levels.

==> eptcsdata.tex <==
\providecommand{\firstpage}{5}
\providecommand{\publicationstatus}{S.-W. Lin and L. Petrucci (Eds.): 2nd French Singaporean\\ Workshop on Formal Methods and Applications\\
EPTCS 156, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.156.5}{10.4204/EPTCS.156.5}}
\pdfoutput=1

